CausalChaos! Dataset for Comprehensive Causal Action Question Answering Over Longer Causal Chains Grounded in Dynamic Visual Scenes

Causal video question answering (QA) has garnered increasing interest, yet existing datasets often lack depth in causal reasoning. To address this gap, we capitalize on the unique properties of cartoons and construct CausalChaos!, a novel, challenging causal Why-QA dataset built upon the iconic "Tom and Jerry" cartoon series. Cartoons use the principles of animation that allow animators to create expressive, unambiguous causal relationships between events to form a coherent storyline. Utilizing these properties, along with thought-provoking questions and multi-level answers (answer and detailed causal explanation), our questions involve causal chains that interconnect multiple dynamic interactions between characters and visual scenes. These factors demand models to solve more challenging, yet well-defined causal relationships. We also introduce hard incorrect answer mining, including a causally confusing version that is even more challenging. While models perform well, there is much room for improvement, especially, on open-ended answers. We identify more advanced/explicit causal relationship modeling & joint modeling of vision and language as the immediate areas for future efforts to focus upon. Along with the other complementary datasets, our new challenging dataset will pave the way for these developments in the field. Project Page: https://github.com/LUNAProject22/CausalChaos

==> Figs/dataset_intro.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cl@{}}
% \toprule
\multicolumn{2}{c}{\textbf{Examples from CausalChaos!}}                                                                                                                                                                                    \\ \midrule
\animategraphics[loop,autoplay,poster=1,width=2cm]{3}{Figs/dataset_intro_frs_indi/1/}{000}{015} 
& 
\raisebox{1cm}{\begin{tabular}[c]{@{}l@{}}Q: Why did Jerry put Tom's tail in the sandwich?\\ A: Jerry wanted Tom to bite his own tail.\\ E: Jerry wanted to inflict pain on Tom.\end{tabular}}                                                         \\ \midrule
\animategraphics[loop,autoplay,poster=1,width=2cm]{3}{Figs/dataset_intro_frs_indi/2/}{000}{015}  
& 
\begin{tabular}[c]{@{}l@{}}Q: Why did Jerry whistle?\\ A: Jerry was whistling for Spike.\\ E: Jerry was calling for Spike to save Jerry from Tom who was about to hit Jerry.\end{tabular}                                              \\
\animategraphics[loop,autoplay,poster=1,width=2cm]{3}{Figs/dataset_intro_frs_indi/3/}{000}{015}  
& 
\begin{tabular}[c]{@{}l@{}}Q: Why was Jerry laughing on the ground?\\ A: Jerry was amused.\\ E: Jerry was amused at Tom whose pants had dropped.\end{tabular}                                                                          \\
\animategraphics[loop,autoplay,poster=1,width=2cm]{3}{Figs/dataset_intro_frs_indi/4/}{000}{015}  
& 
\begin{tabular}[c]{@{}l@{}}Q: Why did Tom put a spoon of hot soup in front of Jerry?\\ A: Tom wanted Jerry to blow at the hot soup.\\ E: Tom thought the soup was too hot and wanted Jerry to help to cool the soup down.\end{tabular} \\ 
% \bottomrule
\end{tabular}
}
% \end{table}

==> Tables/res_oe_consolidated.tex <==
\begin{table*}
\centering
% 
{\input{Tables/res_oe_uniform}
\subcaption*{\textbf{(a)}}}
%
% \bigskip
%
{\input{Tables/res_oe_episodic}
\subcaption*{\textbf{(b)}}}
% 
% \bigskip
% 
{\input{Tables/res_oe_seasonal}
\subcaption*{\textbf{(c)}}}
\vspace{-0.3cm}
\caption{\textbf{OEAG Results} on our dataset. (a) \textbf{UD} split; (b) \textbf{PS} split; (c) \textbf{UN} split.}
\label{tab:res_oe_consolidated}
\end{table*}

==> Tables/res_oe_episodic.tex <==
\resizebox{\textwidth}{!}{%
\small
\centering
\setlength\tabcolsep{5pt}
\begin{tabular}{@{}lccccccccccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} 
 &
  \multicolumn{2}{c}{\textbf{BLEU-1}} &
  \multicolumn{2}{c}{\textbf{BLEU-2}} &
  \multicolumn{2}{c}{\textbf{BLEU-3}} &
  \multicolumn{2}{c}{\textbf{METEOR}} &
  \multicolumn{2}{c}{\textbf{ROUGE}} &
  \multicolumn{2}{c}{\textbf{SPICE}} &
  \multicolumn{2}{c}{\textbf{CIDEr}} &
  \multicolumn{2}{c}{\textbf{S-BERT}} &
  \multirow{2}{*}{\textbf{CapsMIX}}
   \\
      %
   \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} 
   \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}
   %
\multicolumn{1}{c}{} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} \\
 %
   \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} 
   \cmidrule(lr){11-11} \cmidrule(lr){12-12} \cmidrule(lr){13-13} \cmidrule(lr){14-14} \cmidrule(lr){15-15} 
   \cmidrule(lr){16-16} \cmidrule(lr){17-17} \cmidrule(l){18-18}
%
\textbf{BlindQA} \cite{evqa} &
  0.2193 &
  0.1795 &
  0.0772 &
  0.0468 &
  0.0326 &
  0.0149 &
  0.1122 &
  0.0813 &
  0.2501 &
  0.1767 &
  0.2960 &
  0.1147 &
  0.1099 &
  0.0434 &
  0.5129 &
  0.4260 &
  2.6935 \\
\textbf{UATT} \cite{uatt} &
  0.2693 &
  0.1947 &
  0.1257 &
  0.0581 &
  0.0440 &
  0.0146 &
  0.1466 &
  0.0847 &
  0.3226 &
  0.2107 &
  0.3255 &
  0.2012 &
  0.1444 &
  0.0646 &
  0.5364 &
  0.4829 &
  \textbf{3.2260} \\
\textbf{HME} \cite{hme} &
  0.2475 &
  0.1830 &
  0.1031 &
  0.0549 &
  0.0363 &
  0.0154 &
  0.1417 &
  0.0845 &
  0.2820 &
  0.2173 &
  0.2933 &
  0.2549 &
  0.0831 &
  0.0655 &
  0.5165 &
  0.4929 &
  3.0719 \\
\textbf{HGA} \cite{hga} &
  0.2586 &
  0.1842 &
  0.1085 &
  0.0517 &
  0.0365 &
  0.0148 &
  0.1433 &
  0.0932 &
  0.2909 &
  0.1806 &
  0.2908 &
  0.2128 &
  0.0877 &
  0.0266 &
  0.5231 &
  0.4078 &
  2.9111\\ \bottomrule
\end{tabular}%
}

==> Tables/res_oe_seasonal.tex <==
\resizebox{\textwidth}{!}{%
\small
\centering
\setlength\tabcolsep{5pt}
\begin{tabular}{@{}lccccccccccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} 
 &
  \multicolumn{2}{c}{\textbf{BLEU-1}} &
  \multicolumn{2}{c}{\textbf{BLEU-2}} &
  \multicolumn{2}{c}{\textbf{BLEU-3}} &
  \multicolumn{2}{c}{\textbf{METEOR}} &
  \multicolumn{2}{c}{\textbf{ROUGE}} &
  \multicolumn{2}{c}{\textbf{SPICE}} &
  \multicolumn{2}{c}{\textbf{CIDEr}} &
  \multicolumn{2}{c}{\textbf{S-BERT}} &
  \multirow{2}{*}{\textbf{CapsMIX}}
   \\
      %
   \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} 
   \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}
   %
\multicolumn{1}{c}{} &
    \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} \\ 
 %
   \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} 
   \cmidrule(lr){11-11} \cmidrule(lr){12-12} \cmidrule(lr){13-13} \cmidrule(lr){14-14} \cmidrule(lr){15-15} 
   \cmidrule(lr){16-16} \cmidrule(lr){17-17} \cmidrule(l){18-18}
%
\textbf{BlindQA} \cite{evqa} &
  0.2312 &
  0.1847 &
  0.0869 &
  0.0550 &
  0.0319 &
  0.0198 &
  0.1263 &
  0.0930 &
  0.2519 &
  0.1806 &
  0.2758 &
  0.2447 &
  0.0667 &
  0.0265 &
  0.4844 &
  0.4153 &
  2.7747 \\
\textbf{UATT} \cite{uatt} &
  0.2659 &
  0.1936 &
  0.1180 &
  0.0645 &
  0.0548 &
  0.0223 &
  0.1423 &
  0.0868 &
  0.3025 &
  0.2200 &
  0.3449 &
  0.2595 &
  0.0940 &
  0.0713 &
  0.5447 &
  0.4750 &
  3.2601 \\
\textbf{HME} \cite{hme} &
  0.2640 &
  0.1930 &
  0.1238 &
  0.0644 &
  0.0556 &
  0.0239 &
  0.1457 &
  0.0868 &
  0.2998 &
  0.2155 &
  0.3115 &
  0.1623 &
  0.0944 &
  0.0698 &
  0.5341 &
  0.4761 &
  3.1207 \\
\textbf{HGA} \cite{hga} &
  0.2674 &
  0.2293 &
  0.1337 &
  0.0823 &
  0.0620 &
  0.0308 &
  0.1703 &
  0.1123 &
  0.3186 &
  0.2363 &
  0.3734 &
  0.2558 &
  0.1972 &
  0.0477 &
  0.5765 &
  0.4692 &
  \textbf{3.5628} \\ \bottomrule
\end{tabular}%
}

==> Tables/res_oe_uniform.tex <==
\resizebox{\textwidth}{!}{%
\small
\centering
\setlength\tabcolsep{5pt}
\begin{tabular}{@{}lccccccccccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} 
 &
  \multicolumn{2}{c}{\textbf{BLEU-1}} &
  \multicolumn{2}{c}{\textbf{BLEU-2}} &
  \multicolumn{2}{c}{\textbf{BLEU-3}} &
  \multicolumn{2}{c}{\textbf{METEOR}} &
  \multicolumn{2}{c}{\textbf{ROUGE}} &
  \multicolumn{2}{c}{\textbf{SPICE}} &
  \multicolumn{2}{c}{\textbf{CIDEr}} &
  \multicolumn{2}{c}{\textbf{S-BERT}} &
  \multirow{2}{*}{\textbf{CapsMIX}}
   \\
   %
   \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} 
   \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}
   %
 &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
  \textbf{A} &
  \textbf{E} &
   \\ 
%
   \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} 
   \cmidrule(lr){11-11} \cmidrule(lr){12-12} \cmidrule(lr){13-13} \cmidrule(lr){14-14} \cmidrule(lr){15-15} 
   \cmidrule(lr){16-16} \cmidrule(lr){17-17} \cmidrule(l){18-18}
%
\textbf{BlindQA} \cite{evqa} &
  0.2412 &
  0.1912 &
  0.1039 &
  0.0618 &
  0.0415 &
  0.0221 &
  0.1243 &
  0.0891 &
  0.2732 &
  0.1885 &
  0.2956 &
  0.0703 &
  0.1034 &
  0.0403 &
  0.4987 &
  0.4195 &
  2.7646 \\

\textbf{UATT} \cite{uatt} &
  0.2661 &
  0.2203 &
  0.1257 &
  0.0805 &
  0.0575 &
  0.0330 &
  0.1409 &
  0.1046 &
  0.3171 &
  0.2293 &
  0.3547 &
  0.2775 &
  0.1197 &
  0.0397 &
  0.5495 &
  0.4767 &
  3.3928 \\
\textbf{HME} \cite{hme} &
  0.2650 &
  0.2072 &
  0.1301 &
  0.0713 &
  0.0554 &
  0.0219 &
  0.1504 &
  0.0914 &
  0.3125 &
  0.2273 &
  0.3184 &
  0.0826 &
  0.0936 &
  0.0639 &
  0.5328 &
  0.4737 &
  3.0975 \\
\textbf{HGA} \cite{hga} &
  0.2891 &
  0.2263 &
  0.1588 &
  0.0897 &
  0.0789 &
  0.0323 &
  0.1856 &
  0.1130 &
  0.3388 &
  0.2399 &
  0.3980 &
  0.2426 &
  0.2782 &
  0.0573 &
  0.6026 &
  0.4561 &
  3.7872 \\
  
  \textbf{BlindGPT-2} &
  0.3770 &
  0.3165 &
  0.2530 &
  0.1749 &
  0.1632 &
  0.1091 &
  0.2452 &
  0.1761 &
  0.3858 &
  0.2966 &
  0.4305 &
  0.3529 &
  1.2482 &
  0.7690 &
  0.6755 &
  0.6271 &
  6.6006 \\
  
\textbf{VisionGPT-2} &
  0.3878 &
  0.3095 &
  0.2605 &
  0.1727 &
  0.1738 &
  0.1091 &
  0.2560 &
  0.1756 &
  0.3934 &
  0.2941 &
  0.4498 &
  0.3385 &
  1.3725 &
  0.7539 &
  0.6760 &
  0.6350 &
  \underline{6.7582} \\
  
  \midrule

\textbf{BLIP-2} \cite{blip2} &
  0.1381 &
  0.0815 &
  0.0451 &
  0.0256 &
  0.0167 &
  0.0059 &
  0.0664 &
  0.0480 &
  0.1618 &
  0.1312 &
  0.0530 &
  0.0422 &
  0.2279 &
  0.1046 &
  0.3837 &
  0.3614 &
  1.8931 \\

  \textbf{Video-LLaMA} \cite{videollama} &
  0.1241 &
  0.1181 &
  0.0419 &
  0.0344 &
  0.0115 &
  0.0098 &
  0.1477 &
  0.1163 &
  0.1719 &
  0.1435 &
  0.2055 &
  0.1383 &
  0.0836 &
  0.0430 &
  0.5734 &
  0.4834 &
  2.4464 \\

  \textbf{VideoChat2} \cite{videochat2} &
  0.2353 &
  0.2116 &
  0.0823 &
  0.0776 &
  0.0250 &
  0.0253 &
  0.1769 &
  0.1295 &
  0.2667 &
  0.2168 &
  0.3264 &
  0.2547 &
  0.3980 &
  0.2910 &
  0.6445 &
  0.5908 &
  \textbf{3.9524} \\ \bottomrule
\end{tabular}%
}

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


% Include other packages here, before hyperref.
\usepackage{graphicx}
\usepackage{booktabs}

% The "axessiblity" package can be found at: https://ctan.org/pkg/axessibility?lang=en
\usepackage[accsupp]{axessibility}  % Improves PDF readability for those with disabilities.

\usepackage{floatrow}
\usepackage{wrapfig}
\usepackage{moresize}
\usepackage[font={small}]{caption}
\usepackage{numprint}
\usepackage{scalerel}

\usepackage{animate}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{cancel}
\usepackage{soul}
% \usepackage{caption}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{enumitem}
\usepackage[dvipsnames]{xcolor}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
% \newcommand{\TODO}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\supplementary}{\textcolor{RoyalBlue}{Supplementary material}}

%----------quotation box-----------------%
% for adjustwidth environment
\usepackage[strict]{changepage}

% for formal definitions
\usepackage{framed}

% environment derived from framed.sty: see leftbar environment definition
\definecolor{formalshade}{rgb}{0.95,0.95,0.95}

\newenvironment{formal}{%
  \def\FrameCommand{%
    \hspace{1pt}%
    {\color{pink}\vrule width 2pt}%
    {\color{formalshade}\vrule width 4pt}%
    \colorbox{formalshade}%
  }%
  \MakeFramed{\advance\hsize-\width\FrameRestore}%
  \noindent\hspace{-4.55pt}% disable indenting first paragraph
  \begin{adjustwidth}{}{7pt}%
  \vspace{2pt}\vspace{2pt}%
}
{%
  \vspace{2pt}\end{adjustwidth}\endMakeFramed%
}
%---------------------------------------------%
